The Sound of Water: Inferring Physical Properties from Pouring Liquids

We study the connection between audio-visual observations and the underlying physics of a mundane yet intriguing everyday activity: pouring liquids. Given only the sound of liquid pouring into a container, our objective is to automatically infer physical properties such as the liquid level, the shape and size of the container, the pouring rate and the time to fill. To this end, we: (i) show in theory that these properties can be determined from the fundamental frequency (pitch); (ii) train a pitch detection model with supervision from simulated data and visual data with a physics-inspired objective; (iii) introduce a new large dataset of real pouring videos for a systematic study; (iv) show that the trained model can indeed infer these physical properties for real data; and finally, (v) we demonstrate strong generalization to various container shapes, other datasets, and in-the-wild YouTube videos. Our work presents a keen understanding of a narrow yet rich problem at the intersection of acoustics, physics, and learning. It opens up applications to enhance multisensory perception in robotic pouring.

==> figures/containers.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{media/lp50-samples-v1.pdf}
    \caption{
        \textbf{Samples from our LiquidPouring50 dataset.}
        Our dataset contains videos of pouring liquids in
        containers with diverse shapes, materials, opacity
        and background environments.
    }
    \label{fig:sample-cylinder-like}
\end{figure}


==> tables/physical-properties.tex <==
\begin{table}[h]
    \centering
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{llcccccc}
            \toprule
            \textbf{Category}                  & \textbf{Property}              & \textbf{Notation}       & \textbf{Units} & \multicolumn{2}{c}{\textbf{Test set I}} & \multicolumn{2}{c}{\textbf{Test set II}}                                                                                                                                                         \\ \cmidrule{5-8}
            \textbf{}                          & \textbf{}                      & \textbf{}               & \textbf{}      & \textit{Audio-only} $\downarrow$        & \textit{Co-supervised} $\downarrow$                                           & \textit{Audio-only} $\downarrow$ & \textit{Co-supervised} $\downarrow$                                           \\
            \midrule
                                               & Height                         & $H$                     & cm             & 2.23                                    & \cellcolor[HTML]{FFE8E6}2.27  {\footnotesize (\textcolor{red}{-0.04})}        & 2.77                             & \cellcolor[HTML]{FFE8E6}2.85 {\footnotesize (\textcolor{red}{-0.08})}         \\ \cmidrule{2-8}
            \multirow{-2}{*}{\textit{Static}}  & Radius                         & $R$                     & cm             & 1.62                                    & \cellcolor[HTML]{E8FFD9}1.39 {\footnotesize (\textcolor{ForestGreen}{+0.23})} & 2.24                             & \cellcolor[HTML]{E8FFD9}1.88 {\footnotesize (\textcolor{ForestGreen}{+0.36})} \\
            \midrule
                                               & Flow rate                      & $Q(t)$                  & ml/s           & 25.2                                    & \cellcolor[HTML]{E8FFD9}22.5 {\footnotesize (\textcolor{ForestGreen}{+2.80})} & 45.7                             & \cellcolor[HTML]{E8FFD9}40.4 {\footnotesize (\textcolor{ForestGreen}{+5.30})} \\ \cmidrule{2-8}
                                               &                                & $\tau_{\frac{1}{4}}(t)$ & s              & 3.96                                    & \cellcolor[HTML]{FFE8E6}4.16 {\footnotesize (\textcolor{red}{-0.20})}         & 4.39                             & \cellcolor[HTML]{E8FFD9}4.10 {\footnotesize (\textcolor{ForestGreen}{+0.29})} \\
                                               &                                & $\tau_{\frac{1}{2}}(t)$ & s              & 1.62                                    & \cellcolor[HTML]{E8FFD9}1.49 {\footnotesize (\textcolor{ForestGreen}{+0.13})} & 3.44                             & \cellcolor[HTML]{E8FFD9}2.99 {\footnotesize (\textcolor{ForestGreen}{+0.45})} \\
            \multirow{-4}{*}{\textit{Dynamic}} & \multirow{-3}{*}{Time to fill} & $\tau_{\frac{3}{4}}(t)$ & s              & 1.53                                    & \cellcolor[HTML]{E8FFD9}1.07 {\footnotesize (\textcolor{ForestGreen}{+0.46})} & 2.66                             & \cellcolor[HTML]{E8FFD9}2.21 {\footnotesize (\textcolor{ForestGreen}{+0.45})} \\
            \bottomrule
        \end{tabular}%
    }
    \caption{
        \textbf{Improvement by visual co-supervision on estimating physical properties.}
        Mean absolute error in estimating various physical properties.
        Visually co-supervised audio model generally outperforms
        audio-only model in estimating physical properties from pitch.
        Noticeable improvements are reported in estimating radius and
        flow rate. This indicates that co-supervision particularly
        improves estimation of pitch towards the end of the audio as
        well as the slope of pitch generally.
    }
    \label{tab:physical-properties}
\end{table}
% Can remove the +/-
